Certified Roundoff Error Bounds Using Semidefinite Programming

Roundoff errors cannot be avoided when implementing numerical programs with finite precision. The ability to reason about rounding is especially important if one wants to explore a range of potential representations, for instance for FPGAs or custom hardware implementations. This problem becomes challenging when the program does not employ solely linear operations, and non-linearities are inherent to many interesting computational problems in real-world applications. Existing solutions to reasoning possibly lead to either inaccurate bounds or high analysis time in the presence of nonlinear correlations between variables. Furthermore, while it is easy to implement a straightforward method such as interval arithmetic, sophisticated techniques are less straightforward to implement in a formal setting. Thus there is a need for methods which output certificates that can be formally validated inside a proof assistant. We present a framework to provide upper bounds on absolute roundoff errors of floating-point nonlinear programs. This framework is based on optimization techniques employing semidefinite programming and sums of squares certificates, which can be checked inside the Coq theorem prover to provide formal roundoff error bounds for polynomial programs. Our tool covers a wide range of nonlinear programs, including polynomials and transcendental operations as well as conditional statements. We illustrate the efficiency and precision of this tool on non-trivial programs coming from biology, optimization and space control. Our tool produces more accurate error bounds for 23% of all programs and yields better performance in 66% of all programs.

==> defManOcaml.tex <==
%=======================================================================
% Définit le style ssr Gallina pour les listings (Assia Mahboubi 2007)

\lstdefinelanguage{Ocaml} {

% Anything betweeen $ becomes LaTeX math mode
mathescape=true,						
% Comments may or not include Latex commands
texcl=false,


% Vernacular commands
morekeywords=[1]{
Section, Module, End, Require, Import, Export, Defensive, Function,
Variable, Variables, Parameter, Parameters, Axiom, Hypothesis, Hypotheses,
Notation, Local, Tactic, Reserved, Scope, Open, Close, Bind, Delimit,
Definition, Let, Ltac, Fixpoint, CoFixpoint, Morphism, Relation,
Implicit, Arguments, Set, Unset, Contextual, Strict, Prenex, Implicits,
Inductive, CoInductive, Record, Structure, Canonical, Coercion,
Theorem, Lemma, Corollary, Proposition, Fact, Remark, Example,
Proof, Goal, Save, Qed, Defined, Hint, Resolve, Rewrite, View,
Search, Show, Print, Printing, All, Graph, Projections, inside,
outside, Locate, Maximal, assume, procedure, 
Persistent, Digraph, ConcreteBidirectional, G 

},

% Gallina
morekeywords=[2]{match, forall, exists, exists2, fun, fix, cofix, struct,
       as, return, if, is, then, else, begin, end, 
      for,  nosimpl, at,
      
       Noedges, Gp , Fe
      
      },

% Sorts
morekeywords=[3]{Type, Prop},

% Various tactics, some are std Coq subsumed by ssr, for the manual purpose
morekeywords=[4]{ 
         type, let, pose, set, move, case, elim, apply, clear, exception, when, with, of, raise, module,
            hnf, intro, intros, generalize, rename, pattern, after, rec,
	    destruct, induction, using, refine, inversion, injection,
         rewrite, congr, unlock, compute, ring, micromega field,
            replace, fold, unfold, change, cutrewrite, simpl,
         have, suff, wlog, suffices, without, loss, nat_norm,
            assert, cut, trivial, revert, bool_congr, nat_congr,
	 symmetry, transitivity, auto, split, left, right, autorewrite},        

% Terminators
morekeywords=[5]{
         by, done, exact, reflexivity, tauto, romega, omega,
         assumption, solve, contradiction, discriminate},


% Control
morekeywords=[6]{do, last, first, try, idtac, repeat},
keywordsprefix=F
% Various symbols
% For the ssr manual we turn off the prettyprint of formulas
 literate=	
	{->}{{$\rightarrow\,$}}2		
 	{->}{{\tt ->}}3
	{<-}{{$\leftarrow\,$}}2	
 	{<-}{{\tt <-}}2			
 	{>->}{{$\mapsto$}}3		
 	{<=}{{$\leq$}}1			
 	{>=}{{$\geq$}}1		
 	{<>}{{$\neq$}}1
 	{/\\}{{$\wedge$}}2	
 	{\\/}{{$\vee$}}2 		
 	{<->}{{$\leftrightarrow\;$}}3
 	{<=>}{{$\Leftrightarrow\;$}}3
 	{:nat}{{$~\in\mathbb{N}$}}3	
	{fforall\ }{{$\forall_f\,$}}1		
	{forall\ }{{$\forall\,$}}1		
	{exists\ }{{$\exists\,$}}1
 	{negb}{{$\neg$}}1
 	{spp}{{:*:\,}}1
 	{~}{{$\sim$}}1
 	{\\in}{{$\in\;$}}1
 	{/\\}{$\land\,$}1
 	{:*:}{{$*$}}2
	{=>}{{$\,\Rightarrow\ $}}1
 	{=>}{{\tt =>}}2
 	{:=}{{{\tt:=}\,\,}}2
 	{==}{{$\equiv$}\,}2
 	{!=}{{$\neq$}\,}2
 	{^-1}{{$^{-1}$}}1
 	{elt'}{elt'}1
       {=}{{\tt=}\,\,}2
       {+}{{\tt+}\,\,}2,
literate=
	{isn't }{{{\ttfamily\color{dkgreen} isn't }}}1,

% Comments delimiters, we do turn this off for the manual
comment=[s]{(*}{*)},

% Spaces are not displayed as a special character
showstringspaces=false,

% String delimiters
morestring=[b]",
morestring=[d]',

% Size of tabulations
tabsize=3,							

% Enables ASCII chars 128 to 255
extendedchars=true,  		 		

% Case sensitivity
sensitive=true, 

% Automatic breaking of long lines
breaklines=true,

% Default style fors listings
basicstyle=\ttfamily,

% Position of captions is bottom
captionpos=b,							

% Full flexible columns 
columns=fixed,%fullflexible,

% Style for (listings') identifiers
identifierstyle={\ttfamily\color{black}},
% Note : highlighting of Coq identifiers is done through a new
% delimiter definition through an lstset at the begining of the
% document. Don't know how to do better.

% Style for declaration keywords
%keywordstyle=[1]{\ttfamily\color{black}},
keywordstyle=\bfseries,
% Style for gallina keywords
%keywordstyle=[2]{\ttfamily\color{black}},

% Style for sorts keywords
%keywordstyle=[3]{\ttfamily\color{lightblue}},

% Style for tactics keywords
%keywordstyle=[4]{\ttfamily\color{dkblue}},

% Style for terminators keywords
%keywordstyle=[5]{\ttfamily\color{red}},


%Style for iterators
%keywordstyle=[6]{\ttfamily\color{dkpink}},
%keywordstyle=[7]{\ttfamily\color{dkgreen}},
% Style for strings
stringstyle=\ttfamily,

% Style for comments
commentstyle=\rmfamily,

}

%=======================================================================
% Définit le style ssr Gallina pour les listings (Assia Mahboubi 2007)

\lstdefinelanguage{NLCertify} {

% Anything betweeen $ becomes LaTeX math mode
mathescape=true,						
% Comments may or not include Latex commands
texcl=false,


% Vernacular commands
morekeywords=[1]{
Section, Module, End, Require, Import, Export, Defensive, Function,
Variable, Variables, Parameter, Parameters, Axiom, Hypothesis, Hypotheses,
Notation, Local, Tactic, Reserved, Scope, Open, Close, Bind, Delimit,
Definition, Let, Ltac, Fixpoint, CoFixpoint, Morphism, Relation,
Implicit, Arguments, Set, Unset, Contextual, Strict, Prenex, Implicits,
Inductive, CoInductive, Record, Structure, Canonical, Coercion,
Theorem, Lemma, Corollary, Proposition, Fact, Remark, Example,
Proof, Goal, Save, Qed, Defined, Hint, Resolve, Rewrite, View,
Search, Show, Print, Printing, All, Graph, Projections, inside,
outside, Locate, Maximal,
Persistent, Digraph, ConcreteBidirectional, G

},

% Gallina
morekeywords=[2]{match, forall, exists, exists2, fun, fix, cofix, struct,
       as, return, if, is, then, else, begin, end, 
      for,  nosimpl, at,
      
       Noedges, Gp , Fe
      
      },

% Sorts
morekeywords=[3]{Type, Prop},

% Various tactics, some are std Coq subsumed by ssr, for the manual purpose
morekeywords=[4]{ 
         type, let, pose, set, move, case, elim, apply, clear, exception, when, with, of, raise, module,
            hnf, intro, intros, generalize, rename, pattern, after, rec,
	    destruct, induction, using, refine, inversion, injection,
         rewrite, congr, unlock, compute, ring, micromega field,
            replace, fold, unfold, change, cutrewrite, simpl,
         have, suff, wlog, suffices, without, loss, nat_norm,
            assert, cut, trivial, revert, bool_congr, nat_congr,
	 symmetry, transitivity, auto, split, left, right, autorewrite},        

% Terminators
morekeywords=[5]{
         by, done, exact, reflexivity, tauto, romega, omega,
         assumption, solve, contradiction, discriminate},


% Control
morekeywords=[6]{do, last, first, try, idtac, repeat},
keywordsprefix=F
% Various symbols
% For the ssr manual we turn off the prettyprint of formulas
% literate=	
%	{->}{{$\rightarrow\,$}}2		
% 	{->}{{\tt ->}}3
%	{<-}{{$\leftarrow\,$}}2	
% 	{<-}{{\tt <-}}2			
% 	{>->}{{$\mapsto$}}3		
% 	{<=}{{$\leq$}}1			
% 	{>=}{{$\geq$}}1		
% 	{<>}{{$\neq$}}1
% 	{/\\}{{$\wedge$}}2	
% 	{\\/}{{$\vee$}}2 		
% 	{<->}{{$\leftrightarrow\;$}}3
% 	{<=>}{{$\Leftrightarrow\;$}}3
% 	{:nat}{{$~\in\mathbb{N}$}}3	
%	{fforall\ }{{$\forall_f\,$}}1		
%	{forall\ }{{$\forall\,$}}1		
%	{exists\ }{{$\exists\,$}}1
% 	{negb}{{$\neg$}}1
% 	{spp}{{:*:\,}}1
% 	{~}{{$\sim$}}1
% 	{\\in}{{$\in\;$}}1
% 	{/\\}{$\land\,$}1
% 	{:*:}{{$*$}}2
%	{=>}{{$\,\Rightarrow\ $}}1
% 	{=>}{{\tt =>}}2
% 	{:=}{{{\tt:=}\,\,}}2
% 	{==}{{$\equiv$}\,}2
% 	{!=}{{$\neq$}\,}2
% 	{^-1}{{$^{-1}$}}1
% 	{elt'}{elt'}1
%       {=}{{\tt=}\,\,}2
%       {+}{{\tt+}\,\,}2,
literate=
	{isn't }{{{\ttfamily\color{dkgreen} isn't }}}1,

% Comments delimiters, we do turn this off for the manual
comment=[s]{(*}{*)},

% Spaces are not displayed as a special character
showstringspaces=false,

% String delimiters
morestring=[b]",
morestring=[d]',

% Size of tabulations
tabsize=3,							

% Enables ASCII chars 128 to 255
extendedchars=true,  		 		

% Case sensitivity
sensitive=true, 

% Automatic breaking of long lines
breaklines=true,

% Default style fors listings
basicstyle=\ttfamily,

% Position of captions is bottom
captionpos=b,							

% Full flexible columns 
columns=fixed,%fullflexible,

% Style for (listings') identifiers
identifierstyle={\ttfamily\color{black}},
% Note : highlighting of Coq identifiers is done through a new
% delimiter definition through an lstset at the begining of the
% document. Don't know how to do better.

% Style for declaration keywords
keywordstyle=[1]{\ttfamily\color{black}},

% Style for gallina keywords
keywordstyle=[2]{\ttfamily\color{black}},

% Style for sorts keywords
keywordstyle=[3]{\ttfamily\color{black}},

% Style for tactics keywords
keywordstyle=[4]{\ttfamily\color{black}},

% Style for terminators keywords
keywordstyle=[5]{\ttfamily\color{black}},


%Style for iterators
keywordstyle=[6]{\ttfamily\color{black}},
keywordstyle=[7]{\ttfamily\color{black}},
% Style for strings
stringstyle=\ttfamily,

% Style for comments
commentstyle=\rmfamily,

}

